Methodologies for Future Vehicular Digital Twins

The role of wireless communications in various domains of intelligent transportation systems is significant; it is evident that dependable message exchange between nodes (cars, bikes, pedestrians, infrastructure, etc.) has to be guaranteed to fulfill the stringent requirements for future transportation systems. A precise site-specific digital twin is seen as a key enabler for the cost-effective development and validation of future vehicular communication systems. Furthermore, achieving a realistic digital twin for dependable wireless communications requires accurate measurement, modeling, and emulation of wireless communication channels. However, contemporary approaches in these domains are not efficient enough to satisfy the foreseen needs. In this position paper, we overview the current solutions, indicate their limitations, and discuss the most prospective paths for future investigation.

==> Hypothesis.tex <==
\section{Hypothesis}

\begin{itemize}
    \item site specific geometry based models are crucial for vehicular communiation links
\item large number of propagation paths needs to be taken into account (specular and diffuse refelctions)
\item hardware-in-the-loop testing of specific modem realization with radio channel emulators is needed, but commercial hardware is not available on the market
\item 3gpp radio channel models need to be extended to accommodate geoemterical relations to cover vehicular radio links (5G Vehicular, 6G vehicular)
\item Which frequency band to conside -> below 6GHz and mmWave. Similarity between.
\item analyze measurement data to obtain empirical evidence.
\end{itemize}
